Egalitarian ORAM: Wear-Leveling for ORAM

While non-volatile memories (NVMs) provide several desirable characteristics like better density and comparable energy efficiency than DRAM, DRAM-like performance, and disk-like durability, the limited endurance NVMs manifest remains a challenge with these memories. Indeed, the endurance constraints of NVMs can prevent solutions that are commonly employed for other mainstream memories like DRAM from being carried over as-is to NVMs. Specifically, in this work we observe that, Oblivious RAM (ORAM) primitive, the state-ofart solution to tackle memory bus side channel vulnerability, while widely studied for DRAMs, is particularly challenging to implement as-is for NVMs as it severely affects endurance of NVMs. This is so, as the inherent nature of ORAM primitive causes an order of magnitude increase in write traffic and furthermore, causes some regions of memory to be written far more often than others. This non-uniform write traffic as manifested by ORAM primitive stands to severely affect the lifetime of non-volatile memories (1% of baseline without ORAM) to even make it impractical to address this security vulnerability

==> Sec_11_Acknowledgement.tex <==

\section{Acknowledgements}

\label{sec:Acknowledgements}
We thank the anonymous reviews for great suggestions to our paper. We also thank xxxx 's team for helping us collect traces from the 31 workloads. We greatly thank xxx for helping us model a freecursive ORAM controller. 


==> Sec_3_Overview.tex <==
\section{Overview}
\label{sec:overview}
In this section, we will describe the high level overview of \DESIGN. Fig. \ref{fig:WL_flow_chart} shows the algorithm flow chart of \DESIGN. We first choose an ORAM tree size based on the size of PM, block size, and slots per node. Then, we will statically partition the ORAM tree into groups. We also reserve an on-chip 64-bit counter, $Ctr$, to store the number of ORAM accesses performed so far, and initialize it to zero. This is pre-processing. During program execution, for an ORAM access to leaf node $LN$, we shall check the value of $Ctr$. Once $Ctr$ reaches a threshold, $\frac{X}{Z}$, we will trigger \DESIGN, which will determine a group that needs to perform node swaps. We call such node swap most frequently accessed node (MFAN) movement. This completes the wear leveling part. Finally, a node ID translation algorithm is performed to convert logical node IDs to physical node IDs based on the value of $Ctr$. In the following sections, we shall first walk through an example to present the inspiration of \DESIGN. Then, we will describe the partition algorithm to generate groups within an ORAM tree. 
Next, we will introduce our node remapping algorithm, which includes how to perform MFAN movement; which group to perform MFAN movement on; when we decide to perform MFAN movement on a group; and, last but not least, how we retrieve the physical node ID given the logical node ID.
Finally, we will evaluate \DESIGN by showing the performance overhead and lifetime improvement. 


\begin{figure}[t]
    \centering
    \includegraphics[width=.6\linewidth]{Figures/WL_flow_chart.png}
    \caption{Flow chart of \DESIGN.}
    \label{fig:WL_flow_chart}
\end{figure}


